Rapid Structural Pruning of Neural Networks with Set-based Task-Adaptive Meta-Pruning

As deep neural networks are growing in size and being increasingly deployed to more resource-limited devices, there has been a recent surge of interest in network pruning methods, which aim to remove less important weights or activations of a given network. A common limitation of most existing pruning techniques, is that they require pre-training of the network at least once before pruning, and thus we can benefit from reduction in memory and computation only at the inference time. However, reducing the training cost of neural networks with rapid structural pruning may be beneficial either to minimize monetary cost with cloud computing or to enable on-device learning on a resource-limited device. Recently introduced random-weight pruning approaches can eliminate the needs of pretraining, but they often obtain suboptimal performance over conventional pruning techniques and also does not allow for faster training since they perform unstructured pruning. To overcome their limitations, we propose Set-based Task-Adaptive Meta Pruning (STAMP), which task-adaptively prunes a network pretrained on a large reference dataset by generating a pruning mask on it as a function of the target dataset. To ensure maximum performance improvements on the target task, we meta-learn the mask generator over different subsets of the reference dataset, such that it can generalize well to any unseen datasets within a few gradient steps of training. We validate STAMP against recent advanced pruning methods on benchmark datasets, on which it not only obtains significantly improved compression rates over the baselines at similar accuracy, but also orders of magnitude faster training speed.

==> 00A.tex <==

\paragraph{Organization.} The supplementary file is organized as follows: We first describe each component of our Set-based Task-Adaptive Meta-Pruning (STAMP) in detail, including the set encoding function and the set-based structural pruning method (mask generative function) in Section~\ref{sub:set}. Then, in Section~\ref{sub:exps}, we provide the detailed experimental settings and additional results on SVHN using ResNet-18 as the backbone network.


\section{Structural Binary Mask Generation with a Set-encoded Representation}
\label{sub:set}
We now describe how we obtain the set representation with $e(\cdot;\bsy\theta)$ and learn structural pruning masks with the set-based mask generative function $g(\cdot;\bsy\pi)$ introduced in Section~3.2.
\subsection{Set Encoding Function}


%To start with, most network architectures for set input follow encoder-decoder structure to achieve permutation-invariant property. Thus, $e(\tilde{\textbf{X}};\bsy\theta)$ in Equation~\ref{eq:mask-generation} is formulated as below :
%\begin{align}
%\begin{split}
%e(\tilde{\textbf{X}}) = f_{D}(f_{E}(\tilde{\textbf{X}}; \bsy\theta_{E}); \bsy\theta_{D})
%\label{eq:set_func}
%\end{split}
%\end{align}
%where $f_{D}(\cdot; \bsy\theta_{D})$ is arbitrary decoder function and $f_{E}(\cdot; \bsy\theta_{E})$ is arbitrary encoder function. \shorttitle~applies SetTransformer~\cite{lee2018set} module to formulate above equation.

To obtain an optimally pruned neural architecture for the target task, we need to exploit the knowledge of the given task. Conventional pruning schemes search for the desired subnetworks through full mini-batch training, which will incur excessive training cost $\mathcal{C}$ when the data size is large. On the other hand, we rapidly and precisely obtain the desired pruned structures given the encoded reprsentations for each dataset . This procedure of obtaining a set representation $e(\tilde{\textbf{X}};\bsy\theta)$  with the set encoder $e$ parameterized by $\bsy\theta_{(\cdot)}$ is given as follows:
\begin{align}
\begin{split}
e(\tilde{\textbf{X}};\bsy\theta) = f_{D}(f_{E}(\tilde{\textbf{X}}; \bsy\theta_{E}); \bsy\theta_{D})~~~s.t.~~~\tilde{\textbf{X}}\in\mathbb{R}^{B\times X_d} \sim \{\textbf{x}_i\}_{i=1}^N,~\textbf{o}_0=e(\tilde{\textbf{X}};\bsy\theta)\in\mathbb{R}^{r\times X_d}
\label{eq:set_func}
\end{split}
\end{align}
where $\tilde{\textbf{X}}\in\mathbb{R}^{B\times X_d}$ from $\mathcal{D}$ is a sampled task set, $B\leq N$ is the sampled batch, $X_d$ is the input dimensionality, and $r$ is the batch dimension of the set representation ($r\ll B$). We then define the set function as a stacked function of the encoder and the decoder where $f_{E}(\cdot;\bsy\theta_{E})\in\mathbb{R}^{B\times X_d}$ is an arbitrary encoder function parameterized by $\bsy\theta_{E}$ and $f_{D}(\cdot;\bsy\theta_{D})$ is a decoder function parameterized by $\bsy\theta_{D}$. The encoder encodes the sampled task set $\tilde{\textbf{X}}$ and the decoder regenerates the encoded vector to the dataset-level representation. Throughout the paper, we use $r=1$ as the dimension of the set representation. We adopt a transformer module \cite{lee2018set} for set encoding, which is a learnable pooling neural network module with an attention mechanism as shown below:
\begin{align}
\begin{split}
f_E(\cdot)=\mbox{AE}(\mbox{AE}(\cdot)),~~~f_D(\cdot)=\mbox{rF}(\mbox{AE}(\mbox{Pool}_r(\cdot))).
\label{eq:transformer0}
\end{split}
\end{align}
where rF is a fully connected layer, AE is an attention-based block~\cite{vaswani2017attention}, and $\mbox{Pool}_r$ is a Pooling by Multihead Attention with $r$ seed vectors~\cite{lee2018set}. AE is a permutation equivariant block that constructs upon Multi-head attention (MH), introduced in Transformer~\cite{vaswani2017attention}. In other words, AE encodes the set information and consists $f_E(\cdot)$, while $f_D(\cdot)$ also includes AE to model correlation between $r$ vectors after pooling. AE is defined as below:
\begin{align}
\begin{split}
    \mbox{AE}(\cdot) =\mbox{Norm}(H + \mbox{rF}(H))\\
\end{split}
\end{align} 
\begin{align}
\begin{split}
    \mbox{where}~ H= \mbox{Norm} (\cdot + \mbox{MH}(\cdot,\cdot,\cdot))\\
\end{split}
\end{align}
where Norm is layer normalization~\cite{ba2016layer}. The encoder encodes the given dataset using the above module, and the decoder aggregates the encoded vector. The full encoding-decoding process can be described as follows:
\begin{align}
\begin{split}
e(\tilde{\textbf{X}};\bsy\theta) = \mbox{rF}(\mbox{AE}(\mbox{Pool}_r(\mbox{AE}(\mbox{AE}(\tilde{\textbf{X}})))))\in \mathbb{R}^{r\times X_d} 
\end{split}
\end{align}
\begin{align}
\begin{split}
\mbox{where}~ \mbox{Pool}_r(\cdot) = \mbox{AE}(R,\mbox{rF}(\cdot))\in \mathbb{R}^{r\times X_d}
\end{split}
\end{align}
In here, pooling is done by applying multihead attention on a learnable vector $R\in \mathbb{R}^{r\times X_d}$. We set $r=1$ in the experiments to obtain a single set representation vector. By stacking these attention based permutation equivaraint functions, we can obtain the set representation $e(\tilde{\textbf{X}};\bsy\theta)\in \mathbb{R}^{1\times X_d}$ from the sampled task $\tilde{\textbf{X}}\in\mathbb{R}^{B\times X_d} $.

%Now, we calcuate $\textbf{o}_l\in\mathbb{R}^{X_l}$ as introduced in Equation~\ref{eq:mask-generation} and Figure~\ref{fig:method} where $X_l$ is dimension of the activation map. 

%In each layer, we calculate mask by $g_l(\textbf{o}_l;\bsy\pi_l)$ to prune out filters. We first reduce the dimension to $\tilde{\textbf{o}}_l \in\mathbb{R}^{K}$ where $K$ is the number of channels in layer $l$ by average pooling function. Then,  we genearte mask $\textbf{m}_l=g_l(\textbf{o}_l;\bsy\pi_l)$ as below:


%\begin{align}
%\begin{split}
% \bsy\pi_l\sim\prod^K_{k=1}\mbox{beta}(\pi_{l,k};\alpha/K,1)
%\label{eq:set-bbdrop}
%\end{split}
%\end{align}
%\begin{align}
%\begin{split}
% \textbf{m}_l|\bsy\pi_l,\textbf{o}_l\sim\prod^K_{k=1}\mbox{Ber}(m_{l,k};\psi_{l,k}(\gamma_{l,k}\tilde{o}_{l,k} +\beta_{l,k})),~~\mbox{where}~ m_{l,k}\in\{0,1\}
%\label{eq:set-bbdrop-m}
%\end{split}
%end{align}
%\begin{align}
%\begin{split}
%\psi_{l,k}(\cdot)=\pi_{l,k}\mbox{min}(1-\epsilon, \mbox{max}(\epsilon, \cdot)) 
%\label{eq:set-bbdrop-pi}
%\end{split}
%\end{align}

%This Beta-Bernoulli prior and $\beta_{l,k}$ induces sparsity in the generation of the mask and we follow the derivation of BBDropout~\cite{lee2018adaptive} to optimize the approximated posterior by Variational Inference.


\subsection{Mask Generative Function}


%\subsection{Set-dependent Structural Pruning using Sparsity-inducing Prior}
%\label{subsec:structural-pruning}
We now describe the mask generation function $\textbf{m}_l=g_l(\textbf{o}_l;\bsy\pi_l)$ at layer $l$, from which we obtain the pruned model parameter $\bsy\omega_l=\textbf{m}_l\otimes \textbf{W}_l$. %we sample masks from sparsity inducing bayesian prior $\textbf{m}_l\sim{p}(\textbf{m}_l|R(\tilde{\textbf{X}}))$.
%For the meta network $ S $ , 
Similarly as in Lee et al. \cite{lee2018adaptive}, we use the following sparsity-inducing beta-Bernoulli prior to generate a binary pruning mask at each layer, which follows Bernoulli distribution,  \textit{Bernoulli}$(\textbf{m}_l;\bsy\pi_l)$, given the probability of parameterized beta distribution as follows: 
\begin{align}
\begin{split}
\textbf{m}_l|\bsy\pi_l\sim\prod^{C_l}_{c=1}\mbox{Bernoulli}(\mbox{m}_{c,l};\pi_{c,l}),~~~
\mbox{where}~~\bsy\pi_l\sim\prod^{C_l}_{c=1}\mbox{beta}(\pi_{c,l};\alpha_l,1)
\label{eq:bbdrop}
\end{split}
\end{align}
where $C_l$ is the number of channels in layer $l$. With a learnable parameter $\alpha_l$ for the beta distribution, the model learns the optimal binary masks from a randomly sampled value from the beta distribution, to determine which neurons/channels should be pruned. 
We extend this input-independent pruning method to sample binary masks based on the set representation of the target task. This \textit{set-dependent} pruning with STAMP is different from data-dependent BBDropout~\cite{lee2018adaptive} in that the former generates a mask per dataset while the altter generates a mask per instance, which makes it difficult to globally eliminate a channel. Furthermore, rather than searching for the compressed structure by training with mini-batch SGD at each iteration, we utilize a set representation to rapidly obtain a near-optimal subnetwork within a few gradient steps. With the set $e(\tilde{\textbf{X}};\bsy\theta)$ representation obtained from the given dataset $\textbf{X}$, we  calculate the activation $\textbf{o}_l=h_l(\textbf{o}_{l-1};\textbf{W}_l)$ for each layer $l$, where $h_l$ is the function of the layer $l$ (i.e. convolution) and $\textbf{o}_1=h_1(e(\tilde{\textbf{X}};\bsy\theta);\textbf{W}_1)$. We omit the layer notation $l$ for readability in the following equations. Then, we sample a structural pruning mask vector $\textbf{m}$ as follows:
\begin{align}
\begin{split}
\textbf{m}|\bsy\pi,\textbf{o}\sim\prod^{C}_{c=1}\mbox{Bernoulli}(\mbox{m}_c;\pi_c\psi(\gamma_c o_c+\beta_c,\epsilon)),~~~\mbox{s.t.}~~[o_1;...;o_C]=\mbox{Pool}(\textbf{o}_l),
\label{eq:set-bbdrop}
\end{split}
\end{align}
where $\gamma$ and $\beta$ are learnable scaling and shifting factors and Pool is the average pooling for $\textbf{o}$ which obtains a representative value for each channel. The clamping function is defined as $\psi(\cdot,\epsilon)=\mbox{min}(1-\epsilon, \mbox{max}(\epsilon, \cdot))$ with a small $\epsilon>0$. Using a clamping function, the network will retain only the meaningful channels. We employ variational inference to approximate sparsity inducing posterior  $p(\textbf{W},\bsy\pi,\bsy\theta,\bsy\beta|\textbf{X})$. The KL-divergence term for our set-based task-adaptive pruning is as follows:
\vspace{0.1in}
\begin{align}
\begin{split}
D_{KL}[q(\textbf{m},\bsy\pi,\bsy\theta|\textbf{X})\|p(\textbf{m},\bsy\pi,\bsy\theta)] + D_{KL}[q(\bsy\beta)\|p(\bsy\beta)],~~~s.t.~~\bsy\beta\sim\mathcal{N}(\textbf{0},b\textbf{I}),
\label{eq:set-bbdrop-kl}
\end{split}
\end{align}
where $b$ is a fixed value for a variance of the shifting factor $\bsy\beta$ to prevent $\bsy\beta$ from drifting away. The first term can be computed analytically to obtain a closed form solution~\cite{lee2018adaptive,nalisnick2016stick}. Also, we can easily compute the second term, $\mathcal{R(\bsy\omega)}$ in the objective function of \shorttitle~(Equation 2) by updating it with gradient-based methods. %We formulated Equation ~\ref{eq:set-bbdrop-kl}, is adopted from BBdropout~\cite{lee2018adaptive}.


We can further approximate the expectation for the prediction of given dataset $\mathcal{D}$ as follows: %$\{\textbf{x},\textbf{y}\}$:
\begin{align}
\begin{split}
p(\textbf{y}|\textbf{x},\textbf{W},\bsy\theta)\approx p(\textbf{y}|f(\textbf{x};\mathbb{E}_q[\textbf{m}]\otimes\textbf{W},\bsy\theta)),~~~s.t.~~\mathbb{E}_q[\textbf{m}]=\mathbb{E}_q[\bsy\pi]\cdot\psi(\bsy\gamma\mbox{Pool}(\textbf{o})+\bsy\beta,\epsilon)
\label{eq:set-bbdrop-approx}
\end{split}
\end{align}


\section{Experiments}
\label{sub:exps}

\subsection{Experimental Settings}
 We first describe how we meta-train \shorttitle~and set the settings for the baselines , SNIP~\cite{lee2018snip} and MetaPruning~\cite{liu2019metapruning}, for the experiments in the main paper (VGGNet and ResNet-18 on two benchmark CIFAR-10 and SVHN).

For \shorttitle, in \textbf{function} STAMP in Algorithm 1, we update $\bsy\phi=\{\textbf{W},~\bsy\pi,~\bsy\theta\}$ with the learning rate 0.001, 0.01, and 0.001 with Adam optimizer, while decreasing the learning rate by 0.1 at 50\% and 80\% of the total epoch, following the settings of BBDropout~\cite{lee2018adaptive}. For  Algorithm 1, we select $i=2000, B=640$ for VGGNet and $i=3000, B=500$ for ResNet-18. We sampled the same number of instances per class. We further set $N=10$ and the size of the minibatch as $32$. When pruning with \shorttitle, we use the same learning rate as the one we use in the meta training stage for VGGNet. However, for ResNet-18, we set the learning rates as $~\bsy\pi=0.5$ to adjust the pruning rate.

For SNIP~\cite{lee2018snip}, in the ResNet-18 experiment, we do not prune the $1\times1$ convolution layer to match the settings for STAMP experiments. Additionally, we modify the learning rate to 0.01, since at the learning rate of $0.1$, SNIP (P) and SNIP obtained lower accuracies (88.51\% and 85.26\% respectively). For VGGNet, we prune the weights of 16 convolution layers. For SNIP (P) we load the pretrained weights on CIFAR-100 before pruning. 

For MetaPruning~\cite{liu2019metapruning}, we used the same settings for ResNet-18 and ResNet-50 experiments. For VGGNet, we prune filters of 16 convolution layers which is the same as \shorttitle. At the search phase, we search for the architecture under given FLOP constraints. We set the pruning ratio at each layer between 20 \% to 60 \%, to satisfy the FLOP constraints, which is 40 \% to 80 \% for the given setting. For the rest of the experimental settings, we followed the settings in~\cite{liu2019metapruning}.




\subsection{Experimental Results} We report the experimental results on SVHN with ResNet18 in Table~\ref{tab:TAB}, which was omitted from the main paper due to the page limit. We followed the settings of Liu et al.~\cite{liu2017learning} and trained on SVHN for 20 epochs. All other settings are kept the same as the experimental setting in the previous paragraph. The results show that \shorttitle~ has the best trade-off between the accuracy and the efficiency.
\input{00TAB}
\input{00FIG}

STAMP obtains higher accuracy over BBDropout at the same compression rate as shown in Figure~\ref{fig:FIG}). Further, when trained for larger number of epochs, STAMP can obtain even higher accuracy and larger compression rate over BBD as shown in Figure~\ref{fig:FIG}, outperforming all baselines in Table~\ref{tab:TAB}. Although training STAMP for longer epochs yields slightly higher training time than the time required to train the full network, STAMP still trains faster than BBdropout. 


%\input{8_shot}



==> 8_fig.tex <==
\begin{figure}
\vspace{0.1in}
\begin{minipage}{.4\textwidth}
\begin{tabular}{c }
\hspace{-0.2in}
\includegraphics[height=3.3cm]{figures/sup.pdf}\\



%\caption{ \textbf{Accuracy over the ratio of used parameters} for SVHN on ResNet18. \textit{Full} denotes the accuracy of the ResNet18 before pruning.}


\end{tabular}
\end{minipage}
\hspace{-0.7 in}
\begin{minipage}{.65\textwidth}
\footnotesize
\begin{tabular}{l|| c|c|c|c }


\hline 
\multicolumn{1}{l||}{Methods}&\multicolumn{1}{c|}{Accuracy (\%) }&\multicolumn{1}{c|}{P (\%)}&\multicolumn{1}{c|}{FLOPs}&\parbox[c]{1.5cm}{ Training\\Time}\\
\hline \hline
 



Full Network	&
94.57  & 100 & x1.00 & \textbf{0.16 h} \\
%(3913sec)18.5sec
\hline


BBD ($kl$=15)& 94.70 & 11.09 &x2.86& 0.31 h\\

BBD ($kl$=20)& 94.30 & 4.86 &x5.14& 0.31 h\\
BBD ($kl$=25)& 94.12 & 2.71 &x8.62& 0.31 h\\
%(7592sec

\hdashline


STAMP ($K$=1, $kl$=15)&\textbf{ 95.44 } & \textbf{7.83} &x\textbf{4.26} &\textbf{0.11 h} \\
%(2055 sec)

STAMP ($K$=5)&\textbf{ 95.73 } & \textbf{3.84} &x\textbf{6.39} &\textbf{0.19 h} \\
STAMP ($K$=10)&\textbf{ 95.77 } & \textbf{1.81} &x\textbf{8.13} &\textbf{0.31 h} \\

%(2055 sec)






\end{tabular}


\end{minipage}
\vspace{0.1in}
\caption{\small{ \textbf{Left:} Accuracy over the ratio of used parameters for SVHN on ResNet18. \textit{Full} denotes the accuracy of the ResNet18 before pruning. \textbf{Right:} Exploring different $K$ of \shorttitle~ compared with BBDropout~\cite{lee2018adaptive}~(BBD). $kl$ is a scale factor for regularization term. }}
\label{fig:bb}
\vspace{-0.2in}
\end{figure}

==> 8_res.tex <==

\begin{table*}
\tiny
\begin{center}
%\caption{Comparison of model.}
\caption{\small Experiment results of SVHN on ResNet18.  Details are same with the Table~\ref{tab:vgg}. } 
\small
\begin{tabular}{l|| c|c|c|c|c|c }


\hline 
\multicolumn{1}{l||}{Methods}&\multicolumn{1}{c|}{Accuracy (\%) }&\multicolumn{1}{c|}{P (\%)}&\multicolumn{1}{c|}{FLOPs}&\multicolumn{1}{c|}{Training Time }&\multicolumn{1}{c|}{Inference time}&\multicolumn{1}{c}{Expense} \\
\hline \hline
 



Full Network	&
94.57 $\pm$ 0.01 & 100 & x1.00 & 0.16 h & 3.30 sec & 0.24 \$\\
%(3913sec)18.5sec
\hline
Edge-Popup~\cite{ramanujan2019s}	&	
%Edge-Popup (2019)	&
92.61 $\pm$ 0.01 & 5.00 & x1.00& 0.20 h & 6.15 sec &0.29 \$\\ 

SNIP (P)~\cite{lee2018snip}	&	
95.38 $\pm$ 0.01 & 6.06 & x1.00& 0.35 h &6.64 sec &0.51 \$\\ 

SNIP~\cite{lee2018snip}	&	
94.88 $\pm$ 0.01 & 6.06 & x1.00& 0.35 h &6.64 sec &0.51 \$\\   



%SNIP ~\cite{lee2018snip}&	89.60\% $\pm$  &2.0M(18.40\%)&	x1.0&1.80h(6483sec) &1.6sec\\ %29.3sec
%SNIP(Rand) ~\cite{lee2018snip}&	85.16\% $\pm$  &2.0M(18.40\%)&	x1.0&-  &-\\
\hdashline

%[19, 16, 59, 7, 6, 29, 15, 36, 195, 228, 201, 172, 487, 117, 84, 63]
Random Pruned&
 94.39 $\pm$ 0.23 & 72.17 &  x2.99&\textbf{0.08 h} &1.66 sec &\textbf{0.12 \$}\\%1913



MetaPruning~\cite{liu2019metapruning} &
94.49 $\pm$ 0.19 & 70.99 &  x2.83 & 2.41 h  &1.68 sec &3.51 \$\\%	7.8sec 3.2h+

%BBDropout ~\cite{lee2018adaptive} &93.66\% $\pm$ 	&  0.8M(7.49\%)	&  x3.51&37.8sec&1.2sec\\
BBDropout~\cite{lee2018adaptive} & 94.32 $\pm$ 0.02& 4.90 &x5.25& 0.31 h& 1.52 sec & 0.46 \$\\
%(7592sec

\hdashline

STAMP-Structure &\textbf{ 95.17 $\pm$ 0.01}  & \textbf{4.81} &x\textbf{5.47} &\textbf{0.11 h} &\textbf{1.51 sec}  &\textbf{0.16 \$}\\
STAMP&\textbf{ 95.41 $\pm$ 0.01} & \textbf{4.81} &x\textbf{5.47} &\textbf{0.11 h} &\textbf{1.51 sec}  &\textbf{0.16 \$}\\
%(2055 sec)





\end{tabular}
\label{tab:res2}
\vspace{-0.2in}
\end{center}


\end{table*}








==> 8_shot.tex <==

\begin{table*}
\tiny
\begin{center}
%\caption{Comparison of model.}
\caption{\small Exploring different $K$ of \shorttitle~ compared with BBDropout~\cite{lee2018adaptive}~(BBD). $kl$ is a scale factor for regularization term. } 
\small
\begin{tabular}{l|| c|c|c|c }


\hline 
\multicolumn{1}{l||}{Methods}&\multicolumn{1}{c|}{Accuracy (\%) }&\multicolumn{1}{c|}{P (\%)}&\multicolumn{1}{c|}{FLOPs}&\multicolumn{1}{c|}{Training Time }\\
\hline \hline
 



Full Network	&
94.57  & 100 & x1.00 & \textbf{0.168 h} \\
%(3913sec)18.5sec
\hline


BBD ($kl$=15)& 94.70 & 11.09 &x2.86& 0.315 h\\

BBD ($kl$=20)& 94.3 & 4.86 &x5.14& 0.315 h\\
BBD ($kl$=25)& 94.12 & 2.71 &x8.62& 0.315 h\\
%(7592sec

\hdashline


STAMP ($K$=1, $kl$=15)&\textbf{ 95.44 } & \textbf{7.83} &x\textbf{4.26} &\textbf{0.11 h} \\
%(2055 sec)

STAMP ($K$=5)&\textbf{ 95.73 } & \textbf{3.84} &x\textbf{6.39} &\textbf{0.19 h} \\
STAMP ($K$=10)&\textbf{ 95.77 } & \textbf{1.81} &x\textbf{8.13} &\textbf{0. h} \\

%(2055 sec)






\end{tabular}
\label{tab:shot}
\vspace{-0.2in}
\end{center}


\end{table*}







